Neural Networks Against (and For) Self-Training: Classification with Small Labeled and Large Unlabeled Sets

We propose a semi-supervised text classifier based on self-training using one positive and one negative property of neural networks. One of the weaknesses of self-training is the semantic drift problem, where noisy pseudo-labels accumulate over iterations and consequently the error rate soars. In order to tackle this challenge, we reshape the role of pseudo-labels and create a hierarchical order of information. In addition, a crucial step in self-training is to use the classifier confidence prediction to select the best candidate pseudo-labels. This step cannot be efficiently done by neural networks, because it is known that their output is poorly calibrated. To overcome this challenge, we propose a hybrid metric to replace the plain confidence measurement. Our metric takes into account the prediction uncertainty via a subsampling technique. We evaluate our model in a set of five standard benchmarks, and show that it significantly outperforms a set of ten diverse baseline models. Furthermore, we show that the improvement achieved by our model is additive to language model pretraining, which is a widely used technique for using unlabeled documents. Our code is available at https://github.com/p-karisani/RST.

==> doc-ethics.tex <==

\noindent\textbf{Failure mode and potential misuse.} If our model is employed as explained in this article, we expect that it enhances the performance of classifiers in semi-supervised settings. We used five standard benchmarks across various domains to reduce the risk of any bias. Nonetheless, every dataset has a specific data distribution and this can affect the efficacy of any model, including ours.

% If our model is used as described in this paper, we expect that it enhances model performance. We used four datasets across various domains to reduce the risk of any bias. Nonetheless, every domain has a specific data distribution and this can affect the efficacy of active learning algorithms \cite{inactive}.

\noindent\textbf{Privacy.} All the datasets used in our experiments are public and have been recently used in scientific venues. Nonetheless, if one decides to use our model for processing a new task, they should follow the corresponding terms of service. Most importantly, if the task is a social media problem, they should not collect any personal information about users, and should not use our model in sensitive tasks that violate user privacy.

% All the datasets used in our paper are public and have been recently used in NLP venues. The publishers of these datasets have targeted important applications that can benefit the society. Nonetheless, if one decides to use our model for processing a new task, they should follow the corresponding terms of service. Most importantly, they should not collect any personal information about users, or should not use our model in sensitive tasks that violate user privacy.

\noindent\textbf{Costs.} Our model aims at reducing the cost of developing semi-supervised models. Nonetheless, to design our model and to run the baselines, we ran the experiments several dozens of times using a system with a 16 core processor and eight NVIDIA Titan RTX GPUs. Note that in a deployment environment, there is no need to consume such a resource, because our model can be used as is.

% Our model aims at reducing the cost of developing online learning systems. Nonetheless, to design our model and to run the baselines, we ran the experiments several dozens of times using a system with a single core cpu and two NVIDIA Titan RTX GPUs. Note that in a deployment environment, there is no need to consume such a resource and our model can be used as is.

==> doc-method-init.tex <==

In a typical self-training model \cite{self-train}, there is a set $L$ of labeled data, and a set $U$ of unlabeled data. A predictive model is trained on $L$ and is used to probabilistically label $U$. Then, given a hyper-parameter $\theta$, as the minimum confidence threshold, the confidently labeled documents in $U$ and their associated \textit{pseudo-labels} are selected and added to $L$. This procedure is iterative. In this framework, there is no constraint on the choice of the underlying model, except that it is required to assign a confidence score to each pseudo-label. 

There are two challenges to face in this setting:~1)~Self-training suffers from the semantic drift problem \cite{semantic-drift,nell}. That is, as we increase the number of iterations, the error rate accumulates and the class boundaries are distorted. 2)~Neural networks are overconfident in their predictions \cite{neural-conf-0,neural-conf-1}, and as we discuss in Section~\ref{sub-sec:subsample}, this shortcoming deteriorates the quality of the pseudo-labels in each iteration.

To address these challenges, we present Robust Self-Training (\METHOD\!). Algorithm \ref{alg:summary} provides an overview of \METHOD, with two classifiers, in Structured English. Lines \ref{alg-line:self-begins} to \ref{alg-line:self-ends} demonstrate one iteration of the algorithm, which is repeated till the set of unlabeled documents $U$ is exhausted. The iteration begins by initializing the classifiers $C_{1}$ and $C_{2}$. Then, it continues by sampling from the set of pseudo-labels $S$ and distilling it \cite{distill} into the classifier $C_{1}$.\footnote{In the first iteration the set $S$ is empty, therefore, no distillation is done.} Then, another sample from the set of labeled documents~$L$ is taken to further train $C_{1}$ using Equation \ref{eq:loss} (see Section \ref{sub-sec:pretrain}). These steps are re-taken to train the second classifier $C_{2}$. Finally, $C_{1}$ and $C_{2}$ are used in Equation \ref{eq:score} (see Section~\ref{sub-sec:subsample}) to label and score the documents in the set $U$. The top documents are removed from $U$ and are added to the set $S$. Since we have multiple classifiers labeling each document (in this case two classifiers), we store the average of the outputs in $S$. On Line~\ref{alg-line:pretrain}, the entire set~$S$ is used to pretrain the final classifier~$C$, and on Line~\ref{alg-line:finetune}, the set~$L$ is used to finetune~$C$ using Equation~\ref{eq:loss}. In the following two sections we discuss how our algorithm can address the two aforementioned challenges.

\begin{algorithm}
% \setstretch{1.5}
% \algsetup{\scriptsize}
\footnotesize
\caption{Overview of \METHOD}\label{alg:summary}
\begin{algorithmic}[1]
\algrenewcommand\algorithmicindent{7pt}
\Procedure{RST}{}
    \State \textbf{Given:}
    \Indent
        \State $L: \text{Set of labeled documents}$ 
        \State $U: \text{Set of unlabeled documents}$
    \EndIndent
    \State \textbf{Return:}
    \Indent
        \State $\text{Trained classifier on L and U}$
    \EndIndent
    \State \textbf{Execute:}
    \Indent
        \State Set $K$ to 100 // $\text{hyper-parameter (step size)}$
        \State Set $R$ to 70 // $\text{hyper-parameter (sample ratio)}$
        \State Set $S$ to EMPTY // $\text{the set of pseudo-labels}$
        \While{$U$ is not EMPTY}
            \State Initialize \parbox[t]{.7\linewidth}{the classifiers $C_{1}$ and $C_{2}$}\label{alg-line:self-begins}
            \State Sample \parbox[t]{.7\linewidth}{$R\%$ of $S$ and use it to train $C_{1}$}
            \State Sample \parbox[t]{.7\linewidth}{$R\%$ of $L$ and use in Equation \ref{eq:loss} for $C_{1}$}
            \State Sample \parbox[t]{.7\linewidth}{$R\%$ of $S$ and use it to train $C_{2}$}
            \State Sample \parbox[t]{.7\linewidth}{$R\%$ of $L$ and use in Equation \ref{eq:loss} for $C_{2}$}
            \State Use $C_{1}$ \parbox[t]{.7\linewidth}{and $C_{2}$ to label $U$ and then score the documents using Equation \ref{eq:score}}
            \State Remove \parbox[t]{.7\linewidth}{the top $K$ documents from $U$ and add them to $S$}
            \EndWhile\label{alg-line:self-ends}
        \State Use the set $S$ to train the classifier $C$\label{alg-line:pretrain}
        \State Use the set $L$ in Equation \ref{eq:loss} to further train $C$\label{alg-line:finetune}
        \State \textbf{Return} $C$
    \EndIndent
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-0.2cm}

\vspace{-0.2cm}
\subsection{Overcoming Semantic Drift} \label{sub-sec:pretrain}
An inherent pitfall of the self-training algorithm is the semantic drift problem \cite{semantic-drift,nell,semantic-drift-solution}, where adding new pseudo-labels ultimately impacts the properties of the classes in the set of labeled documents. 
% This typically results in a shift from a high precision model to a high recall model. 
To mitigate this problem, one solution is to use the set of pseudo-labels as the secondary source of information\footnote{One can also reduce the importance of the pseudo-labels, which we use as a baseline.}--instead of augmenting it with the set $L$. Thus, we seek to re-design self-training such that it accommodates a hierarchical order of information.

Catastrophic forgetting is a problem in neural networks \cite{catastrophic-1, catastrophic-2}. This problem arises in the continual learning settings, when a series of tasks are sequentially used to train a neural network. It stems from the fact that the weights of the neural network update to serve the objective of the current task, therefore, the information about the current task replaces the information about the previous tasks. Thus, if the neural network is \textit{carefully} trained for the current task, one may be able to construct a natural hierarchical order of information in the network. Based on this argument, we propose to use the set of pseudo-labels to initialize the network in each iteration, and then, further train using the set $L$ of labeled data.\footnote{The method proposed in this section does not add computational complexity to the regular neural self-training. We discuss the computational complexity in Appendix~\ref{sec:appendix-resource}.}

To be able to initialize and train the network in each iteration, we store two sets of documents. The set $S$ that contains the pseudo-labeled documents collected from the previous self-training iterations, and the set $L$ that contains the initial labeled documents. At the beginning of each iteration, we use the documents in $S$ to train the network, i.e., Task~1. We store--and use--the last layer logits of the network in classifying the documents in $S$ to be used with a high temperature for initialization.\footnote{See the article by \citet{distill} for the role of high temperature in model distillation.} Thus, we essentially distill the knowledge of the previous iterations into the network \cite{distill}. Then, we use the documents in $L$ and minimize the following objective function to further train the network, i.e., Task~2:
\begin{equation} \label{eq:loss}
\small
\setlength{\jot}{0pt}
\setlength{\abovedisplayskip}{6pt}
\setlength{\belowdisplayskip}{6pt}
\medmuskip=0mu
\thinmuskip=0mu
\thickmuskip=0mu
\nulldelimiterspace=0pt
\scriptspace=0pt
\begin{split}
\mathcal{L}= &(1-\lambda)(-\sum_{i=1}^{N}[y_{i}\log a_{i}+(1-y_{i})\log (1-a_{i})]) + \\ 
&\lambda(-\sum_{i=1}^{N}[q_{i}\log a'_{i}+(1-q_{i})\log (1-a'_{i})]),
\end{split}
\end{equation}
where $N$ is the number of the documents in the set $L$, $y_{i}$ is the binary ground truth label of the document $d_{i}$, $a_{i}$ is the output of the network after the softmax layer, $a'_{i}$ is the output of the network after the softmax layer with a high temperature \cite{distill}, and $q_{i}$ is the output of the network with the same temperature as the previous case right before the current task begins. Note that $a'_{i}$ and $q_{i}$ are different, the former refers to the current output of the network, while the weights are still being updated to meet the objective of the current task, and the latter refers to the output of the network after it was trained by the documents in the set $S$ and before it was trained by the documents in the set $L$. $\lambda$ is a penalty term ($0 \leq \lambda \leq 1$).

The first term in the loss function is the regular cross entropy between the ground truth labels and the output class distributions. The second term is the cross entropy between the current output class distributions and the class distributions that were obtained after training the network by the pseudo-labels. Intuitively, the goal of the second term is to prevent the first term from fully erasing the knowledge already stored in the network, i.e., the knowledge obtained from the pseudo-labels.

% There is a resemblance between Equation \ref{eq:loss} and the equation proposed in \cite{distill} for aggregating the hard and soft labels in the distillation process. However, unlike the equation in the distillation process, the second term in our objective function is not to distill knowledge into the network, but to protect the already stored knowledge from being overwritten.

One advantage of employing pseudo-labels to initialize the network, as we described in this section, is that if during the self-training iterations due to the growing size of the set $S$ the newly added pseudo-labels become highly noisy, the first term in the objective function yields stronger gradients and will automatically dampen the effect of these examples. In fact, we show that given this mechanism, there is no need to validate the number of self-training iterations anymore, and one can label and use the entire set $U$. Whereas, doing so in the regular self-training causes semantic drift.

The idea proposed in this section is related to two separate lines of work in the machine learning literature: 1) The research on pretraining neural network models: \citet{pretraining} convincingly show that pretraining a model with closely related labeled data, i.e., training the model before the actual task begins improves model robustness. Their experiments justify the utility of network initialization. No previous work exists on the applicability of this mechanism to semi-supervised learners, where labeled data is small and only unlabeled in-domain data is available. We are the first to utilize the pretraining/finetuning paradigm in training such learners. 2) The studies on curriculum learning: \citet{curriculum} show that the order of training examples can impact the quality of the local minima in non-convex optimization problems, e.g., in training a neural network. The authors base their idea on the properties of training examples, whereas, the order of examples in our model is determined by the nature of labels.

\vspace{-0.2cm}
\subsection{Addressing Overconfidence} \label{sub-sec:subsample}
The performance in each self-training iteration heavily depends on the quality of the pseudo-labels added to the training data in the previous iterations. Neural networks are prone to assigning high posterior probabilities even to the out of distribution data points \cite{neural-conf-1}. This means, with a high probability, the mislabeled documents can be confidently assigned to the opposite class and can be selected as the best candidate documents. The effect of these spurious labels can accumulate over iterations and eventually deteriorate the performance.\footnote{Throttling is used to reduce this effect \cite{semiupervised-nlp-book}, which we use in the experiments. Our solution specifically reduces the noise introduced by an overconfident model.}

To address this issue, in this section we propose a novel selection criterion to replace the plain confidence metric. Our criterion takes into account the uncertainty in the classifier output. The core idea of our algorithm is to determine whether the output class distributions of a candidate document under multiple different subsamples of the set $L$ are consistent.\footnote{In terms of runtime and memory consumption our model is comparable to existing semi-supervised learning models. In fact, three of our baselines consist of model ensembling (they use two or more classifiers), which is a common practice in semi-supervised learning. We discuss this in Appendix~\ref{sec:appendix-resource}.} A small divergence--while having distinctly different training sets--indicates that there are strong similarities between the candidate document and the set $L$. A high confidence that occurs due to the poor calibration of neural network outputs, and not because of the qualities of data, is less likely to re-occur under multiple sample sets.

% To address this issue, we propose to \textit{subsample} two sets from the set $L$ in each iteration--with replacement and preserving the original class distributions. Then, train two \textit{identical} networks\footnote{In terms of runtime and memory consumption our model is comparable to existing semi-supervised learning models. In fact, three of our baselines consist of model ensembling (they use two or more classifiers), which is a common practice in semi-supervised learning. We discuss this in Appendix~\ref{sec:appendix-resource}.} on each subset, and use them to label the documents in the set $U$. The best candidate documents in $U$ are the ones that confidently classified by the two networks and have low overall uncertainty.

% % The best candidate documents in $U$ are the ones that are confidently classified by the two networks, and also, have the same output class distributions under the two settings.

% Note that this, perhaps misleadingly nostalgic, algorithm has subtle reasoning and interpretation. The logic behind this algorithm is to determine whether the output class distributions of a candidate document under two different subsamples of the set $L$ are consistent. We keep the two classifiers identical in order to make an effort to uncover the reason behind the divergence between two classifier outputs. A small divergence--while keeping the two classifiers identical and having distinctly different training sets--indicates that there are strong similarities between the candidate document and the set $L$. A high confidence that occurs due to the poor calibration of neural network outputs, and not because of the qualities of data, is less likely to re-occur under two different sample sets.

% From a different perspective, our method can have an uncertainty-based interpretation. Our algorithm can be seen as a method for measuring the epistemic uncertainty in the model \cite{uncertainty}. Because fixing the model and sampling from the training set essentially enables us to quantify the divergence in the predictions under two data availability settings. Thus, our algorithm inherently incorporates the prediction uncertainty into the selection metric.

To implement this idea, we note that the selection criterion must be proportional to model confidence and disproportional to output uncertainty. Below we propose a metric that follows our desired criteria:

% \begin{equation} \label{eq:score}
% % \small
% % \setlength{\jot}{0pt}
% % \setlength{\abovedisplayskip}{6pt}
% % \setlength{\belowdisplayskip}{6pt}
% % \medmuskip=0mu
% % \thinmuskip=0mu
% % \thickmuskip=0mu
% % \nulldelimiterspace=0pt
% % \scriptspace=0pt
% \begin{split}
% Score(d)=\frac{(1 - \hat{H}(a_{1})) \times (1 - \hat{H}(a_{2})) + \alpha }{JS(P_{a_{1}} \left|\right| P_{a_{2}}) + \alpha},
% \end{split}
% \end{equation}

\begin{equation} \label{eq:score}
\small
\setlength{\jot}{0pt}
\setlength{\abovedisplayskip}{6pt}
\setlength{\belowdisplayskip}{6pt}
\medmuskip=0mu
\thinmuskip=0mu
\thickmuskip=0mu
\nulldelimiterspace=0pt
\scriptspace=0pt
\begin{split}
Score(d)=\frac{\prod_{i=1}^{m}(1 - \hat{H}(P_{a_{i}})) + \alpha }{GJS(P_{a_{1}}, \dots ,P_{a_{m}}) + \alpha},
\end{split}
\end{equation}

where $d$ is the candidate document; $P_{a_{i}}$ is the output distribution of the classifier $C_{i}$ trained on the \textit{i-th} subsample; $\hat{H}(a_{i})$ is the normalized entropy of the class distribution; $GJS$ is the generalized Jensen-Shannon distance between the class distributions $P_{a_{1}}, \dots, P_{a_{m}}$; $m$ is the number of subsamples---in Algorithm \ref{alg:summary} $m$ equals 2---; and $\alpha$ is a smoothing factor---we set it to \num{1e-4} in all the experiments. Depending on the value of $\alpha$, the equation results in $Score(d)\in(0,+\infty)$.

The normalized entropy \cite{n-entropy} of a random variable is the entropy of the random variable divided by its maximum entropy:
\begin{equation} \nonumber
\small
\setlength{\jot}{0pt}
\setlength{\abovedisplayskip}{6pt}
\setlength{\belowdisplayskip}{6pt}
\medmuskip=0mu
\thinmuskip=0mu
\thickmuskip=0mu
\nulldelimiterspace=0pt
\scriptspace=0pt
\begin{split}
\hat{H}(X) = -\sum_{}^{n} p(X) \frac{\log~p(X)}{\log~n},
\end{split}
\end{equation}
where $n$ is the number of classes. We use the normalized variant instead of the regular Shannon entropy to scale the quantity between 0 and 1. The generalized Jensen-Shannon distance \cite{gjs} measures the diversity between a set of distributions, and is calculated as follows:
% \begin{equation} \nonumber
% \small
% \setlength{\jot}{0pt}
% \setlength{\abovedisplayskip}{6pt}
% \setlength{\belowdisplayskip}{6pt}
% \medmuskip=0mu
% \thinmuskip=0mu
% \thickmuskip=0mu
% \nulldelimiterspace=0pt
% \scriptspace=0pt
% \begin{split}
% JS(P\left|\right|Q)=\sqrt{\frac{KL(P\left|\right|Q)+KL(Q\left|\right|P)}{2}},
% \end{split}
% \end{equation}
% where $KL$ is the Kullback-Leibler divergence between the two distributions $P$ and $Q$. 

\begin{equation} \nonumber
\small
\setlength{\jot}{0pt}
\setlength{\abovedisplayskip}{6pt}
\setlength{\belowdisplayskip}{6pt}
\medmuskip=0mu
\thinmuskip=0mu
\thickmuskip=0mu
\nulldelimiterspace=0pt
\scriptspace=0pt
\begin{split}
GJS(P_{a_{1}}, \dots ,P_{a_{m}})=H(\overline{P})-\frac{1}{m} \sum_{i=1}^{m} H(P_{a_{i}}),
\end{split}
\end{equation}

where $H(\parm)$ is the Shannon entropy, and $\overline{P}$ is the mean of the distributions. The mean is calculated as follows:

\begin{equation} \nonumber
\small
\setlength{\jot}{0pt}
\setlength{\abovedisplayskip}{6pt}
\setlength{\belowdisplayskip}{6pt}
\medmuskip=0mu
\thinmuskip=0mu
\thickmuskip=0mu
\nulldelimiterspace=0pt
\scriptspace=0pt
\begin{split}
\overline{P}=\frac{1}{m} \sum_{i=1}^{m} P_{a_{i}}.
\end{split}
\end{equation}

The numerator in Equation \ref{eq:score} represents the confidence of the classifiers. Higher confidence in the classification yields lower entropy in the class predictions, and hence, results in a higher score. The denominator in Equation \ref{eq:score} represents the output uncertainty. Using Equation \ref{eq:score} we can score the documents in the set $U$, and select the top documents and their associated pseudo-labels to be added to the set $L$--we assume all classifiers agree on the labels of the top candidate documents.\footnote{We did not observe an example that violates this assumption in the experiments. Nonetheless, such an example can be taken as noise and can be discarded.}
% \textbf{Distinctions between our model and existing ensemble methods.} There are three differences between our model and existing ensemble classifiers: 1) Existing models rely primarily on classifier confidence scores to select top candidate documents, which is inefficient when the underlying model is a neural network. 2) There is no uncertainty interpretation provided for existing models. 3) Existing ensemble models use multiple classifiers for prediction during the test phase. Whereas, we use only one classifier during test phase, which is more resource efficient. 
In Section~\ref{subsec:main-results}, we compare our method with several ensemble models and show that it ranks first. Additionally, in Section~\ref{subsec:analysis}, we compare our method with a variant of an ensemble classifier that uses output entropy to further support the efficacy of our approach.

% Intuitively, we try to measure the amount of shared information between the labeled and unlabeled data, instead of relying on the confidence of the model, to select the best candidates. We achieve this by ensuring that the unlabeled documents have the same output class distributions under multiple random subsets of the training set, eliminating the sole reliance on the confidence of the classifier.

% The idea proposed in this section is inspired by the early works of Riloff and her colleagues on using extraction patterns for Information Extraction in a bootstrapping algorithm \cite{bootstrap-1,bootstrap-2}. In the cited articles, the authors use the amount of shared information between the labeled and unlabeled data, instead of relying on the confidence of the model, to select the best candidates. In our case, since neural networks rely on the distributional representations, we achieve the same goal by ensuring that the unlabeled documents have the same output class distributions under multiple random subsets of the training set, eliminating the sole reliance on the confidence of the classifier.

So far we discussed binary classification problems. Extending our method to multi-class tasks is trivial. To do so, we only need to replace the binomial cross entropy in Equation \ref{eq:loss} with a multinomial cross entropy. Note that Equation \ref{eq:score} remains intact, because it is agnostic to the number of classes. 

% \textbf{A note on utility of self-training framework.} Given the numerous methods of regularization and generalization in neural networks \cite{VAT,UDA}, the utility of a self-training framework can be called into question. However, a self-training model should not be taken as the only and ultimate solution in the low-data regime. While this technique is employed, the data perturbation \cite{VAT} or augmentation \cite{UDA,var-pretrain} methods can be also utilized. The pseudo-ensembling models \cite{pseudo-ensemble,dropout} can be further added. The domain specific pretraining can be performed \cite{bert,do-pretrain}, and the available domain knowledge \cite{co-decomp} can be incorporated. 

% In the next section, we outline the details of our experiments.

% \subsection{Computational Complexity} \label{sub-sec:resource}

% During the experiments, we observed that even with two subsamples our model outperforms existing baselines. Therefore, we used only two classifiers in all the experiments. In terms of implementation, our model has two variants: a sequential variation and a parallel variation. In the sequential setting, the classifier $C_{1}$ is trained on the sets $S$ and $L$, and then it is used to label the set $U$. The pseudo-labels are stored and the classifier is removed from the memory. This process is repeated for the classifier $C_{2}$ to obtain the second set of pseudo-labels. The two sets of pseudo-labels are processed using Equation 1, and the sets $S$ and $U$ are updated. In this setting, the memory footprint is identical to that of the regular self-training and the run-time is $2\times$ slower; because each iteration involves training both networks. In the parallel setting, both classifiers $C_{1}$ and $C_{2}$ can be trained at the same time to obtain the sets of pseudo-labels. In this case, our model has $2\times$ more parameters, because both networks should be stored in memory. Since in the parallel case the two networks do not communicate, the run-time is significantly shorter than the sequential case--it is easily comparable to that of the regular self-training. 

% In our experiments, we used NVIDIA Titan RTX GPUs--this GPU has 24 GB memory. We used the sequential variation of our model. On average, our model took up less than 10 GB of memory and was fully trained in less than 3 hours with the 10,000 unlabeled documents in each dataset.




